Thompson's group T has quadratic Dehn function

We prove that Thompson's group $T$ and, more generally, all the Higman-Thompson groups $T_n$ have quadratic Dehn function.

==> custom-commands.tex <==
\RequirePackage{xspace}
\RequirePackage{amsthm,amssymb,amsmath,amsfonts}
\RequirePackage{mathtools}
\RequirePackage{etoolbox}
\RequirePackage{tikz-cd}
\RequirePackage{hyperref}
\RequirePackage[capitalize]{cleveref}
\RequirePackage{tabularray}

\renewcommand{\epsilon}{\varepsilon}

\newcommand\emptyarg{{}\cdot{}}


\DeclarePairedDelimiterX\norm[1]\lVert\rVert{
	\ifblank{#1}{\emptyarg}{#1}
}
\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
	\ifblank{#1}{\emptyarg}{#1}
}

\DeclarePairedDelimiterX\scalar[2]\langle\rangle{
	\ifblank{#1}{\emptyarg}{#1}, \ifblank{#2}{\emptyarg}{#2}
}

\DeclarePairedDelimiter\set\{\}

\DeclarePairedDelimiter\lclosed{[}{)}
\DeclarePairedDelimiter\rclosed{(}{]}

\DeclarePairedDelimiter\cardinality\lvert\rvert


\newcommand\restrict[2]{{%
\left.\kern-\nulldelimiterspace %
#1 %
\vphantom{|} %
\right|_{#2} %
}}

\newcommand{\into}{\hookrightarrow}

\newcommand{\onto}{\twoheadrightarrow}

\newcommand\bigfun[5]{%
	\begin{tikzcd}[
			column sep=2em,
			row sep=1ex,
			ampersand replacement=\&
		]
		#1\colon \&[-3em]
		#2\vphantom{#3} \arrow[r] \&
		#3\vphantom{#2} \\
		\&
		#4\vphantom{#5}  \arrow[r,mapsto] \&
		#5\vphantom{#4}
	\end{tikzcd}%
}

\newcommand{\composed}{\circ}

\def\coloneq{\coloneqq}


\NewDocumentCommand{\ZZ}{o}{\IfNoValueTF{#1}{\mathbb Z}{\mathbb Z/#1\mathbb Z}}

\newcommand{\NN}{\mathbb N}

\newcommand{\QQ}{\mathbb Q}

\newcommand{\RR}{\mathbb R}

\newcommand{\HH}{\mathbb H}

\newcommand{\positive}[1]{#1^+}
\newcommand{\negative}[1]{#1^-}
\newcommand{\nonpositive}[1]{#1_{\leq 0}}
\newcommand{\nonnegative}[1]{#1_{\geq 0}}

\NewDocumentCommand{\tuple}{m O{1} m}{#1_#2, \dots, #1_#3}

\NewDocumentCommand{\range}{O{1} m}{%
	\ifthenelse{\equal{#1}{1} \AND \equal{#2}{3}}{%
		\set{1,2,3}%
	}{%
		\ifthenelse{\equal{#1}{1} \AND \equal{#2}{2}}{%
			\set{1,2}%
		}{%
			\set{#1, \dots, #2}%
		}%
	}
}




\newcommand\generatedby[1]{\presentation{#1}{}}

\DeclarePairedDelimiterX\presentation[2]\langle\rangle{
	#1 \ifblank{#2}{}{| #2}
}

\DeclareMathOperator{\Area}{Area}

\newcommand{\quotient}[2]{#1/#2}
\newcommand{\lquotient}[2]{#1\backslash#2}

\newcommand{\Dehn}[1]{\delta_{#1}}
\newcommand{\asympleq}{\preccurlyeq}
\newcommand{\asympgeq}{\succcurlyeq}

\let\acts\curvearrowright

\newcommand{\CAT}[1]{\ensuremath{\operatorname{CAT}(#1)}\xspace}


\newcommand{\conj}[2]{\inv{#2}#1#2}
\newcommand{\Conj}[2]{\Inv{#2}#1#2}

\NewDocumentCommand{\finitetype}{o}{\ensuremath{\IfValueTF{#1}{\mathcal F_#1}{\mathcal F}}\xspace}


\NewDocumentCommand{\shortexactsequence}{m O{} m O{} m}{
	\begin{tikzcd}[ampersand replacement=\&]
		1 \arrow[r] \& #1 \arrow[r, "#2"] \& #3 \arrow[r, "#4"] \& #5 \arrow[r] \& 1
	\end{tikzcd}
}


\newcommand{\isom}{\cong}

\newcommand{\qi}{\cong_{\operatorname{QI}}}



\newcommand{\boundary}{\partial}

\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\ball}[2]{B_#1(#2)}

\newcommand{\skel}[2]{#2^{(#1)}}

\DeclareMathOperator{\sd}{sd}

\newcommand{\barycentre}[1]{\hat{#1}}

\newcommand{\regneigh}[1]{N(#1)}

\newcommand{\univcov}[1]{\widetilde{#1}}

\newcommand{\lift}[1]{\tilde{#1}}

\NewDocumentCommand{\sphere}{m}{S^#1}
\NewDocumentCommand{\Hyp}{m}{\mathbb H^#1}

\newcommand{\transpose}[1]{\leftindex^t #1}
\newcommand{\inv}[1]{#1^{-1}}
\DeclarePairedDelimiterXPP{\Inv}[1]{}(){^{-1}}{#1}

\newcommand{\model}[1][\kappa]{\ensuremath{\mathcal M_{#1}}}

\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Homeo}{Homeo}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\image}{Im}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\interior}{Int}
\DeclareMathOperator{\Sol}{Sol}
\DeclareMathOperator{\coflink}{cof\hspace{0cm}Lk}
\DeclareMathOperator{\flink}{f\hspace{0cm}Lk}
\DeclareMathOperator{\link}{Lk}
\NewDocumentCommand{\linkup}{o m}{\link_\uparrow(#2 \IfValueT{#1}{;#1})}
\NewDocumentCommand{\linkdown}{o m}{\link_\downarrow(#2 \IfValueT{#1}{;#1})}
\NewDocumentCommand{\flinkup}{o m}{\flink_\uparrow(#2 \IfValueT{#1}{;#1})}
\NewDocumentCommand{\flinkdown}{o m}{\flink_\downarrow(#2 \IfValueT{#1}{;#1})}
\NewDocumentCommand{\coflinkup}{o m}{\coflink_\uparrow(#2 \IfValueT{#1}{;#1})}
\NewDocumentCommand{\coflinkdown}{o m}{\coflink_\downarrow(#2 \IfValueT{#1}{;#1})}
\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\subdivision}{sd}


\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{corollary}[lemma]{Corollary}
\theoremstyle{remark}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{notation}{Notation}
\theoremstyle{definition}
\newtheorem{definition}[lemma]{Definition}
\newcounter{MainTheorems}
\renewcommand{\theMainTheorems}{\Alph{MainTheorems}}
\newtheorem{maintheorem}[MainTheorems]{Theorem}

\crefformat{enumi}{#2\textup{(#1)}#3}
\crefmultiformat{enumi}{#2\textup{(#1)}#3}{,~#2\textup{(#1)}#3}{,~#2\textup{(#1)}#3}{ and~#2\textup{(#1)}#3}

\newcommand{\newterm}[1]{\emph{#1}}

\newcommand{\strong}[1]{\textbf{#1}}

